Pod-Deployability in Kubernetes with Inter-Pod Affinity Constraints is PSPACE-Complete

Kubernetes is the de-facto platform for container orchestration. Its scheduler combines resource capacities with label-based affinity and anti-affinity rules, and the interaction of these features can make the eventual placement of a pod. In this paper, we study the pod-deployability problem: given an initial cluster, a pod type, and a designated node, does some legal sequence of pod deployments and deletions cover the target pair? We give three complexity results. First, when dynamic constraints contain no affinity (anti-affinity is allowed), pod-deployability is decidable in polynomial time. Second, required affinity together with required anti-affinity makes the problem PSPACE-complete. Third, required affinity alone is already enough for PSPACE-completeness on a single node with one scalar capacity. The lower bounds encode, respectively, 1-safe Petri-net coverability and bounded black pebbling. These results isolate two independent sources of state-space complexity in Kubernetes scheduling: logical exclusion and resource-bounded prerequisite management.

==> macros.tex <==
\usepackage[
  disable,     %
  %
  %
  %
  textwidth=\marginparwidth,
  colorinlistoftodos,
  prependcaption,
  linecolor=green,backgroundcolor=green!25,bordercolor=green
  ]{todonotes}
\makeatletter
\if@todonotes@disabled
\else %
\newlength{\increase}
\setlength{\increase}{8cm}
\paperwidth=\dimexpr \paperwidth + \increase\relax
\oddsidemargin=\dimexpr\oddsidemargin + .5\increase\relax
\evensidemargin=\dimexpr\evensidemargin + .6\increase\relax
\marginparwidth=\dimexpr \marginparwidth + .4\increase\relax
\let\tmptitle\title
\renewcommand{\title}[1]{\tmptitle{#1{\tiny\normalfont \makebox[10em]{\colorbox{red!20}{disable todos}}}}}
\fi
\makeatother

\makeatletter
\def\blfootnote{\gdef\@thefnmark{}\@footnotetext}
\makeatother

\usepackage{amsmath,amssymb,mathtools,booktabs}
\usepackage{stmaryrd}
\usepackage{cleveref}
\usepackage[subtle]{savetrees}
\usepackage{tikz}
\usetikzlibrary{arrows.meta,positioning,shapes.geometric,fit,decorations.pathreplacing}

\newcommand{\PodTypes}{\mathcal T}
\newcommand{\Nodes}{\mathcal N}
\newcommand{\Resources}{\mathcal R}
\newcommand{\used}{\mathsf{used}}
\newcommand{\StaticOK}{\mathsf{StaticOK}}
\newcommand{\Hard}{\mathsf{Hard}}
\newcommand{\Aff}{\mathsf{Aff}}
\newcommand{\Anti}{\mathsf{Anti}}
\newcommand{\Deploy}{\mathsf{Deploy}}
\newcommand{\sem}[1]{\llbracket#1\rrbracket}
\newcommand{\zero}{\mathbf 0}
\newcommand{\PSPACE}{\mathsf{PSPACE}}
\newcommand{\polytime}{\mathsf{P}}
\setlength{\emergencystretch}{2em}

